Implicit-explicit, realizability-preserving first-order scheme for moment models with Lipschitz-continuous source terms

We derive an implicit-explicit (IMEX), realizability-preserving first-order scheme for moment models with Lipschitz-continuous source terms. In contrast to fully-explicit schemes the time step does not depend on the physical parameters, removing the stiffness from the system. Furthermore, a wider class of collision operators (e.g. the Laplace-Beltrami operator) can be used. The derived scheme is applied to minimum-entropy models.

==> Sections/DG.tex <==
\section{Discontinuous-Galerkin scheme}

We consider a usual first-order system of hyperbolic balance laws
\begin{align}
\label{eq:GeneralHyperbolicSystem1D}
\dt\moments+\dz\Flux\left(\moments\right) = \Source\left(\moments\right),
\end{align}
where $\moments(\timevar,\x)\in\R^{\momentnumber}$ for all $\timevar\in\timeint$ and $\x\in\Domain$.

In the following, the spatial domain $\Domain = (\zL, \zR)$ is divided into (for notational simplicity) $\ncells$ (equidistant) cells $\cell{\cellind} = (\z_{\cellind-\frac12}, \z_{\cellind+\frac12})$, where the cell interfaces are given by $\z_{\cellind\pm\frac12} = \z_\cellind \pm 
\frac{\dzstepsize}{2}$ for cell centres $\z_\cellind = \zL + (\cellind - \frac12)\dzstepsize$, and
$\dzstepsize = \frac{\zR - \zL}{\ncells}$. 

Furthermore, $\SpaceOfPolynomials{\spatialorder}(\cell{\cellind})$ is the set of polynomials of degree at most $\spatialorder$ on the interval $\cell{\cellind}$, and 
\begin{equation}
\FiniteElementSpace{\spatialorder} = \{\Testfunction \in \Lp{1}(\Domain): \Testfunction|_{\cell{\cellind}} \in \SpaceOfPolynomials{\polydegree}(\cell{\cellind}) \text{ for } 
 \cellind \in \{ 1, \ldots , \ncells \} \}
\label{eq:dg-space}
\end{equation}
is the finite-element space of piecewise polynomials of degree $\polydegree$.\\

The discontinuous-Galerkin method for the general hyperbolic system \eqref{eq:GeneralHyperbolicSystem1D}, as outlined in \cite{Cockburn1989,Cockburn1989a,Cockburn1991}, can be briefly described as follows.

For each $\timevar\in\timeint$, seek an approximate solution $\momentsprojected(\timevar, \z)$ whose components live in the finite-element space $\FiniteElementSpace{\spatialorder}$ as defined in \eqref{eq:dg-space}.

Then follow the Galerkin approach: replace $\moments$ in \eqref{eq:GeneralHyperbolicSystem1D} by a 
solution of the form $\momentsprojected \in \FiniteElementSpace{\spatialorder}$, multiply the resulting equation by basis functions $\Testfunction[h]$ of $\FiniteElementSpace{\spatialorder}$ and integrate over cell $\cell{\cellind}$ to obtain
\begin{subequations}
\label{eq:dweakform1}
\begin{align}
 \dt \int_{\cell{\cellind}} \momentsprojected(\timevar, \z)\Testfunction[h](\z)~d\z
 &+ \Flux(\momentsprojected(\timevar, \z_{\cellind+\frac12}^-)) \Testfunction[h](\z_{\cellind+\frac12}^-)
  - \Flux(\momentsprojected(\timevar, \z_{\cellind-\frac12}^+)) \Testfunction[h](\z_{\cellind-\frac12}^+) \nonumber \\
 &-\int_{\cell{\cellind}} \Flux(\momentsprojected(\timevar, \z)) \dz \Testfunction[h](\z)~d\z 
 = \int_{\cell{\cellind}} \Source(\momentsprojected(\timevar, \z))\Testfunction[h](\z)~d\z  \label{eq:dweakform1a},\\
 \int_{\cell{\cellind}} \momentsprojected(0, \z)\Testfunction[h](\z)~d\z &= \int_{\cell{\cellind}} \momentstzero(\z) 
\Testfunction[h](\z)~d\z,
 \label{eq:dweakform1b}
\end{align}
\end{subequations}
where $\z_{\cellind \pm \frac12}^-$ and $\z_{\cellind \pm \frac12}^+$ again denote the limits 
from left and right, respectively, and $\momentstzero$ is the initial condition. 
In order to approximately solve the Riemann problem at the cell-interfaces,
the fluxes $\Flux(\momentsprojected(\timevar, \z_{\cellind + \frac12}^\pm))$ at the points of discontinuity are both replaced by a 
numerical flux $\numericalFlux(\momentsprojected(\timevar, \z_{\cellind+\frac12}^-), \momentsprojected(\timevar, \z_{\cellind+\frac12}^+))$, thus 
coupling the elements with their neighbours \cite{Toro2009}. Several well-known examples for such a numerical flux $\numericalFlux$ exist in literature. The simplest example is the global Lax-Friedrichs flux
\begin{align}
\label{eq:globalLF}
 \numericalFlux(\moments[1], \moments[2]) = \dfrac{1}{2} \left( \Flux(\moments[1]) + \Flux(\moments[2]) - C ( \moments[2] - 
 \moments[1]) \right).
\end{align}
The numerical viscosity constant $\viscosityconstant$ is taken as the global estimate of the 
absolute value of the largest eigenvalue of the Jacobian
$\Flux'$. 

The local Lax-Friedrichs flux could be used instead.
This requires computing the eigenvalues of the Jacobian in every
space-time cell to adjust the value of the numerical viscosity constant $\viscosityconstant$
but possibly decreases the overall diffusivity of the scheme.
However, since high-order methods are considered, the decrease in
diffusivity achieved by switching to the local Lax-Friedrichs flux should be
negligible.\\

The usual approach is to expand the approximate solution $\momentsprojected$ on each interval as
\begin{align}
\label{eqn:solution_form}
\left.\momentsprojected\right|_{\cell{\cellind}}(\timevar, \z) := \momentslocal{\cellind}(\timevar, \z) := \sum_{\polybasisind=0}^{\polydegree}\momentspolynomialcoefficients{\cellind}{\polybasisind}(\timevar) 
\Testfunction[\polybasisind]\left( \frac{\z - \z_\cellind}{\dzstepsize} \right),
\end{align}
where $\Testfunction[0], \Testfunction[1], \ldots ,\Testfunction[\polydegree]$ denote a 
basis for $\SpaceOfPolynomials{\spatialorder}(\referencecell)$ with respect to the standard $\Lp{2}$-scalar product on the reference cell $\referencecell = \left(-\frac12,\frac12\right)$. It is convenient to choose an orthogonal basis like the Legendre 
polynomials scaled to the interval $\referencecell$, denoted by
\begin{align}
\label{eq:LegendrePolynomialBasis}
\Testfunction[0](\referencevar) = 1, \quad \Testfunction[1](\referencevar) = 2\referencevar, \quad \Testfunction[2](\referencevar) = 
 \frac12 (12\referencevar^2-1), \: \ldots
\end{align}
With an orthogonal basis the cell means $\momentscellmean{\cellind}$ are easily available from the 
expansion coefficients $\momentspolynomialcoefficients{\cellind}{\polybasisind}$, since
$$
\momentscellmean{\cellind}(\timevar) := \frac{1}{\dzstepsize} \int_{\cell{\cellind}} \momentslocal{\cellind}(\timevar, \z)~d\z
 = \frac{1}{\dzstepsize} \sum_{\polybasisind=0}^{\polydegree} \momentspolynomialcoefficients{\cellind}{\polybasisind}(\timevar)
 \int_{\cell{\cellind}} \Testfunction[\polybasisind]\left( \frac{\z-\z_\cellind}{\dzstepsize} \right)~d\z
 = \momentspolynomialcoefficients{\cellind}{0}(\timevar).
$$
Collecting the coefficients $\momentspolynomialcoefficients{\cellind}{\polybasisind}(\timevar)$ into the $\spatialorder \times 
\momentnumber$ matrix
$$
\momentspolynomialmatrix{\cellind}(\timevar) = \left( \momentspolynomialcoefficients{\cellind}{0}(\timevar),\ldots , \momentspolynomialcoefficients{\cellind}{\polydegree}(\timevar)\right)^T,
$$

equation \eqref{eq:dweakform1} can be written in compact form as the coupled system of ordinary differential equations
\begin{align}
\label{eq:odeDG}
\dt \momentspolynomialmatrix{\cellind} &= \DifferentialOperatorLocal(\momentspolynomialmatrix{\cellind - 1}, \momentspolynomialmatrix{\cellind}, \momentspolynomialmatrix{\cellind + 1}), \quad 
\text{for } 
\cellind \in \{1, \ldots , \ncells\} \text{ and } \timevar \in \timeint,
\end{align}
with initial condition \eqref{eq:dweakform1b} and an appropriate choice of the local differential operator $\DifferentialOperatorLocal$.

We incorporate boundary conditions via `ghost cells' at $\z_0$ and $\z_{\ncells+1}$ and set $\momentslocal{0}(\timevar, \z)$ and $\momentslocal{\ncells + 1}(\timevar, \z)$ accordingly.

For Dirichlet-boundary conditions, the simplest approach is taken. The ghost-cell values are chosen to be the constant functions 
\begin{align*}
\momentslocal{0}(\timevar, \z) &\equiv \momentslocal{0}(\timevar, \z_{\frac12})\momentslocal{0}(\timevar, \z_{\frac12}),\\
\momentslocal{\ncells + 1}(\timevar, \z) &\equiv \momentslocal{\ncells + 1}(\timevar, \z_{\ncells + \frac12}),
\end{align*}
with $\momentslocal{0}(\timevar, \z_{\frac12})$ and $\momentslocal{\ncells + 1}(\timevar, \z_{\ncells + \frac12})$ defined by the boundary conditions.\\

For periodic boundary conditions, the obvious choice is
\begin{align*}
\momentslocal{0}(\timevar, \z) &= \momentslocal{\ncells}(\timevar, \z+\zR-\zL),\quad \z\in\cell{0},\\
\momentslocal{\ncells + 1}(\timevar, \z) &=\momentslocal{1}(\timevar, \z-\zR+\zL),\quad \z\in\cell{\ncells+1}.
\end{align*}

To obtain a high-order scheme for \eqref{eq:odeDG} a suitable time integrator has to be used. Such a class of integrators is given by the \emph{strong-stability-preserving} (\emph{SSP}) methods, as used for example in \cite{Zhang2010,AllHau12}. The
stages and steps of these type of methods are convex combinations of forward-Euler steps.
Since the realizable set is convex, the analysis of a forward-Euler step
then suffices to prove realizability preservation of the high-order method.\\

When possible, \emph{SSP-Runge-Kutta} (\emph{SSP-RK}) methods are used, but unfortunately they only exist up to order four \cite{Ruuth2004,Gottlieb2005}.
For higher orders the so-called \emph{two-step Runge-Kutta} (\emph{TSRK}) \emph{SSP}
methods \cite{Ketcheson2011} as well as their generalizations, the
\emph{multi-step Runge-Kutta} (\emph{MSRK}) \emph{SSP} methods \cite{Bresten2013} can be applied.
They combine Runge-Kutta schemes with positive weights and
high-order multistep methods to achieve a total order higher than
four while maintaining the important SSP property.

See \cite{Schneider2015b} for more information about the SSP-schemes used in the actual implementation. 

In this work we want to investigate different combinations of troubled-cell indicators $\tcindicator$ and slope limiters/reconstructors $\slopelimiter$.
In general, the process of limiting will be denoted by 

\begin{align}
\label{eq:slopelimiterscalar}
\momentspolynomialmatrix{\cellind} 
= 
\begin{cases}
\slopelimiter(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder})  & \text{ if } \tcindicator(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder}) = 1\\
\momentspolynomialmatrix{\cellind} & \text{otherwise}.
\end{cases}
\end{align}

It has been found that applying the limiter to the components 
themselves may introduce non-physical oscillations around an otherwise monotonic 
solution \cite{Cockburn1989}.
Instead, the limiter is applied to the local characteristic fields of the 
solution. They are found by transforming the vector $\moments$ 
using the matrix $\eigenvectormatrix_{\cellind}$, whose columns hold the eigenvectors of the Jacobian 
$\Flux'(\momentscellmean{\cellind})$ evaluated at the cell mean $\momentscellmean{\cellind}$.
After applying the limiter, the characteristic fields are transformed back to the conserved quantities.
In the end, since $\momentspolynomialmatrix{\cellind}$ is a matrix of size $\spatialorder \times \momentnumber$, this transformation is accomplished by post-multiplying with $\eigenvectormatrix_{\cellind}^{-T}$ 
so that
\begin{align}
\label{eq:DGLimiter}
 \slopelimitercf(\momentspolynomialmatrix{\cellind-1},\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+1}) = \slopelimiter(\momentspolynomialmatrix{\cellind-1}\eigenvectormatrix_{\cellind}^{-T},\momentspolynomialmatrix{\cellind}\eigenvectormatrix_{\cellind}^{-T},\momentspolynomialmatrix{\cellind+1}\eigenvectormatrix_{\cellind}^{-T})\eigenvectormatrix_{\cellind}^T,
\end{align}
and similarly for $\tcindicator$.

In the following we will neglect the transformation to characteristic fields for notational simplicity.

\subsection{WENO reconstruction and smoothness indicators}

\subsection{Troubled-cell indicators}
\comment{blabla}

\subsubsection{TVBM-corrected minmod indicator}
\label{sec:TVBMminmod}
An often-used indicator is the \emph{TVBM-corrected minmod limiter} proposed in
\cite{Cockburn1989a}. It assumes that the major part of the spurious oscillations is generated in the linear part of the underlying polynomial, whose slope in the reference cell is simply $\momentspolynomialcoefficients{\cellind}{1}$.

The indicator in the $\cellind^{\text{th}}$ cell is then given by
\begin{align}
\tcindicator(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder})
= 
\begin{cases}
1 & \text{ if }
     \abs{\momentspolynomialcoefficients{\cellind}{1}} \geq \TVBconstant(\dzstepsize)^2 \text{ and } \minmod{\momentspolynomialcoefficients{\cellind}{1}, \momentspolynomialcoefficients{\cellind+1}{0} - \momentspolynomialcoefficients{\cellind}{0}, 
                  \momentspolynomialcoefficients{\cellind}{0} - \momentspolynomialcoefficients{\cellind-1}{0}} \neq \momentspolynomialcoefficients{\cellind}{1},\\
0 &\text{otherwise}.                 
\end{cases}
% \slopelimiter(\momentspolynomialmatrix{\cellind-1},\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+1}) = \left\{ 
%  \begin{array}{cc}
%   \left( \begin{array}{c}
%           \left( \momentspolynomialcoefficients{\cellind}{0} \right)^T \\
%            \minmod{\momentspolynomialcoefficients{\cellind}{1}, \momentspolynomialcoefficients{\cellind+1}{0} - \momentspolynomialcoefficients{\cellind}{0}, 
%             \momentspolynomialcoefficients{\cellind}{0} - \momentspolynomialcoefficients{\cellind-1}{0}}^T \\
%           (0, 0, \ldots , 0)\\
%           \vdots\\
%           (0, 0, \ldots , 0)
%          \end{array} \right)
%    &\text{ if }
%     \abs{\momentspolynomialcoefficients{\cellind}{1}} \geq \TVBconstant(\dzstepsize)^2, \\     
%    \momentspolynomialmatrix{\cellind} & \text{otherwise},
%  \end{array} \right.
\end{align}
%for the $\cellind^{\text{th}}$ cell and the case $\spatialorder \geq 3$, that is piece-wise quadratic or higher-degree polynomials, so that the final rows of zeros in the first case indicates
%that the coefficients for the higher-order basis functions are set to zero for
%each component.
The absolute value and the inequality are applied componentwise. %The label ``scalar'' is used because the limiter is directly applied to each 
%scalar component of $\momentscollection{}$.
The function $\minmod{\cdot}$ is the standard minmod function applied componentwise, defined by
\begin{align}
\label{eq:minmod}
\minmod{a_1,a_2,a_3} &= \begin{cases}
 \operatorname{sign}(a_1) \min\{|a_1|,|a_2|,|a_3|\} & \text{if } 
 \operatorname{sign}(a_1) = \operatorname{sign}(a_2) = 
 \operatorname{sign}(a_3), \\
0 & \text{else}.
\end{cases}
\end{align}

The constant $\TVBconstant$ is a problem-dependent estimate of the second derivative, 
though it has to be noted that in \cite{Cockburn1989a} the authors did not find the 
solutions very sensitive to the value chosen for this parameter.


\subsection{Slope limiters and reconstructors}
\comment{bla}
\subsubsection{The minmod limiter}
Often-used due to its simplicity and small stencil is the following limiter
\begin{align*}
\slopelimitercf(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder})
= 
\left( \begin{array}{c}
\left( \momentspolynomialcoefficients{\cellind}{0} \right)^T \\
\minmod{\momentspolynomialcoefficients{\cellind}{1}, \momentspolynomialcoefficients{\cellind+1}{0} - \momentspolynomialcoefficients{\cellind}{0}, 
\momentspolynomialcoefficients{\cellind}{0} - \momentspolynomialcoefficients{\cellind-1}{0}}^T \\
                             (0, 0, \ldots , 0)\\
                             \vdots\\
                             (0, 0, \ldots , 0)
                            \end{array} \right)
\end{align*}
for the case $\spatialorder \geq 3$, that is piece-wise quadratic or higher-degree polynomials, so that the final rows of zeros in the first case indicates that the coefficients for the higher-order basis functions are set to zero for each component. As before, the minmod function is defined as in \eqref{eq:minmod}.

This limiter has the known disadvantage that it reduces the accuracy at smooth extrema for that it is mostly combined with the TVBM-corrected minmod indicator as in \secref{sec:TVBMminmod} which does not identify smooth extrema as troubled if the constant $\TVBconstant$ is chosen correctly. 

Note that there are generalizations of this indicator and limiter combination like in \cite{Krivodonova2007} which are not investigated here.

\subsection{WENO}
\comment{begin bla}
Here, the standard WENO reconstruction method given for example in \cite{Shu1998,Toro2009} is used.
For the unfamiliar reader, the method is introduced briefly in this section,
while a more detailed documentation\footnote{Most of the documentation and the code has been written by Jochen Kall.} and demo implementations of the
used reconstruction procedures can be found on the web page
\cite{AGTMWENOpage}. Note that the described techniques should in principle work with every accurate high-order polynomial reconstruction method.\\

Since it is not a priori clear what it means to do a polynomial reconstruction in space of a function in angle, the angular domain has to be discretized using the quadrature rule $\angularQuadrature$ (see \secref{sec:QRealizability}). Then, the following techniques can be applied at every quadrature point $\angularQuadratureNodes{\angularQuadratureIndex}$. For clarity of exposition, the time dependence is suppressed here.\\

Given polynomials of degree $\polydegree$, $\WENOpoly{\cellind}{\WENOind}(\cdot, \SCheight) \in \SpaceOfPolynomials{\polydegree}\left(\cell{\cellind}\right)$, $\WENOind = 0, 1, \ldots , \spatialorder$, each solving the interpolation problem
\begin{equation}
 \cellmean[\cellindvar]{\WENOpoly{\cellind}{\WENOind}(\z, \SCheight)} =  \distributioncellmean{\cellind}(\SCheight),
  \qquad \cellindvar \in \WENOstencil{\cellind}{\WENOind}{\spatialorder} := \{\cellind - \spatialorder + \WENOind, \ldots ,  \cellind + \WENOind - 1\},
\label{eq:interpolation}
\end{equation}
the WENO method then calculates coefficients $\WENOweights^{\pm}_{\cellind-\frac12, \WENOind}$
to form the weighted averages
$$
\WENOpoly{\cellind}{-\frac12}^\pm(\z, \SCheight) := \sum_{\WENOind = 0}^\spatialorder
 \WENOweights^{\pm}_{\cellind-\frac12, \WENOind} \WENOpoly{\cellind}{\WENOind}(\z, \SCheight).
$$

The set $\WENOstencil{\cellind}{\WENOind}{\spatialorder}$ is called the \emph{WENO stencil} of order $\spatialorder$ in cell $\cellind$ with shift $\WENOind$. The weights $\WENOweights^{\pm}_{\cellind-\frac12, \WENOind}$ are non-linear functions
of the cell-averages and reflect the smoothness of each polynomial $\WENOpoly{\cellind}{\WENOind}$. 
They are computed such that for smooth data the approximation order at the 
cell edge is maximized.
This gives an order $2 \spatialorder - 1$ approximation at the cell interface, while
the overall order in the interior of the cell is $\spatialorder$.

When at least one of the interaction coefficients $\absorption$ or
$\scattering$ is spatially dependent, it is necessary to specify the reconstruction
inside each cell. Thus it is essential to make a choice, because both $\WENOpoly{\cellind}{\mp \frac12}^\pm$
are order $\spatialorder$ reconstructions of the density $\ansatz$ in the $\cellind^{\text{th}}$ cell%
\footnote{
Some reconstruction methods, such as sub-cell WENO \cite{Cheng2013} or minmod \cite{Toro2009},
give only one polynomial reconstruction inside each cell, and so for these
methods such a choice would be unnecessary.
}.
\comment{end bla}

==> Sections/realizability.tex <==
\section{Realizability}

Since the underlying kinetic density to be approximated is
non-negative, a 
moment vector only makes sense physically if it can be associated with a 
non-negative distribution function. In this case the moment vector is called 
\emph{realizable}.

\begin{definition}
\label{def:RealizableSet}
The \emph{realizable set} $\RD{\basis}{}$\index{Realizability@\textbf{Realizability}!Realizable set $\RD{\basis}{}$} is 
$$
\RD{\basis}{} = \left\{\moments~:~\exists \distribution(\SCheight)\ge 0,\, \momentcomp{0} = \ints{\distribution} > 0,
 \text{ such that } \moments =\ints{\basis\distribution} \right\}.
$$
If $\moments\in\RD{\basis}{}$, then $\moments$ is called \emph{realizable}.
Any $\distribution$ such that $\moments =\ints{\basis \distribution}$ is called a \emph{representing 
density}. If $\distribution$ is additionally a linear combination of Dirac deltas \cite{Hassani2009,Mathematics2011,Kuo2006}, it is called \emph{atomic} \cite{Curto1991}.
\end{definition}
\begin{remark}
\mbox{ }
\begin{enumerate}[(a)]
\item The realizable set is a convex cone, and
\item Representing densities are not necessarily unique.
\end{enumerate}
\end{remark}
%

Additionally, since the entropy ansatz has the form \eqref{eq:psiME}, in the 
Maxwell-Boltzmann case, the optimization problem \eqref{eq:primal} only has a 
solution if the moment vector lies in the ansatz space
$$
 \AnsatzSpace := \left\{\ints{\basis \ansatz[\moments]}\stackrel{\eqref{eq:psiME}}{=} \ints{\basis \ld{\entropy}'\left(\basis^T\multipliers\right) }
  : \multipliers \in \R^{\momentnumber}  \right\}.
$$
In the case of a bounded angular domain, the ansatz 
space $\AnsatzSpace$ is equal to the set of realizable moment vectors 
\cite{Jun00}. Therefore, it is sufficient to focus on realizable moments only.

Unfortunately, the definition of the realizable set is not constructive, making it hard to check if a moment vector is realizable or not. Therefore, other characterizations of $\RD{\basis}{}$ are necessary.

For example, in the classical mixed-moment problem of first order, the realizable set is characterized by the inequalities \cite{Frank07,Schneider2014}
\begin{align*}
\momentcomp{1+}-\momentcomp{1-}\leq \momentcomp{0} \quand \pm \momentcomp{1\pm}\geq 0.
\end{align*}

In this paper, we want to focus on the lowest-order non-trivial model of the differentiable mixed-moment hierarchy, i.e. $\momentorder = 2$.

\begin{theorem}
The moment vector $\moments = \left(\momentcomp{0},\momentcomp{1},\momentcomp{2+},\momentcomp{2-}\right)\in\R^4$ is realizable, i.e. $\moments\in\RD{\basis}{}$, if and only if
\begin{align}
\label{eq:Realizability1D}
%\normalizedmomentcomp{2+} - \sqrt{\normalizedmomentcomp{2-}\, \left(1-\normalizedmomentcomp{2+}\right)} &\leq \normalizedmomentcomp{1} \leq \sqrt{\normalizedmomentcomp{2+}\, \left(1-\normalizedmomentcomp{2-}\right)} - \normalizedmomentcomp{2-}\\
\momentcomp{2+} - \sqrt{\momentcomp{2-}\, \left(\momentcomp{0}-\momentcomp{2+}\right)} &\leq \momentcomp{1} \leq \sqrt{\momentcomp{2+}\, \left(\momentcomp{0}-\momentcomp{2-}\right)} - \momentcomp{2-}\\
\momentcomp{0},\momentcomp{2\pm}\geq 0. \label{eq:Realizability1Db}
%\normalizedmomentcomp{2+}+\normalizedmomentcomp{2-}\geq \normalizedmomentcomp{1}^2
%\momentcomp{0}\left(\momentcomp{2+}+\momentcomp{2-}\right)\geq \momentcomp{1}^2 \label{eq:Realizability1Db}
\end{align}
\end{theorem}
\begin{proof}
At first, we want to show that \eqref{eq:Realizability1D} and \eqref{eq:Realizability1Db} are necessary. Assume that $\distribution\geq 0$ is arbitrary but fixed. Note that $\momentcomp{0\pm}\geq \pm\momentcomp{1\pm}\geq \momentcomp{2\pm}\geq 0$ and $\momentcomp{0\pm}\momentcomp{2\pm}\geq \momentcomp{1\pm}^2$ due to the half-moment realizability conditions \cite{Schneider2014,Curto1991}. Then we have (using $\momentcomp{0-}+\momentcomp{0+} = \momentcomp{0}$) that 
\begin{align*}
\momentcomp{2-}\, \left(\momentcomp{0}-\momentcomp{2+}\right) = \momentcomp{2-}\momentcomp{0-}+ \momentcomp{2-}\left(\momentcomp{0+}-\momentcomp{2+}\right) \geq \momentcomp{1-}^2 + \momentcomp{2-}\left(\momentcomp{0+}-\momentcomp{2+}\right) \geq \momentcomp{1-}^2.
\end{align*}
Since $\momentcomp{1-}\leq 0$ it follows that 
\begin{gather*}
\sqrt{\momentcomp{2-}\, \left(\momentcomp{0}-\momentcomp{2+}\right) } \geq \abs{\momentcomp{1-}} = -\momentcomp{1-}\\
\Leftrightarrow\\
-\sqrt{\momentcomp{2-}\, \left(\momentcomp{0}-\momentcomp{2+}\right) } \leq \momentcomp{1-}.
\end{gather*}
Therefore 
\begin{align*}
\momentcomp{2+} - \sqrt{\momentcomp{2-}\, \left(\momentcomp{0}-\momentcomp{2+}\right)} \leq \momentcomp{2+}+\momentcomp{1-} \leq \momentcomp{1+}+\momentcomp{1-} = \momentcomp{1}.
\end{align*}
The upper bound can be shown to be necessary in a similar way.\\
\eqref{eq:Realizability1Db} follows from the positivity of $1$ and $\SCheight^2$. We want to remark that the standard second-order full-moment realizability condition for $\momentcomp{2} = \momentcomp{2+}+\momentcomp{2-}$, namely $\momentcomp{0}\left(\momentcomp{2+}+\momentcomp{2-}\right)\geq \momentcomp{1}^2$, is implied by \eqref{eq:Realizability1D}+\eqref{eq:Realizability1Db}. 

To show that the above inequalities are also sufficient, we provide a non-negative realizing distribution with support in $[-1,1]$:
\begin{align*}
\distribution = \momentcomp{0}\left(\cfrac{\normalizedmomentcomp{1+}^2}{\normalizedmomentcomp{2+}}\cdot\dirac\left(\SCheight-\cfrac{\normalizedmomentcomp{2+}}{\normalizedmomentcomp{1+}}\right)+\cfrac{\normalizedmomentcomp{1-}^2}{\normalizedmomentcomp{2-}}\cdot\dirac\left(\SCheight-\cfrac{\normalizedmomentcomp{2-}}{\normalizedmomentcomp{1-}}\right)\right),
\end{align*}
with
\begin{align*}
\normalizedmomentcomp{1+} = \frac{\normalizedmomentcomp{2+}\, \left(\normalizedmomentcomp{1} + \normalizedmomentcomp{2-}\, \sqrt{\frac{ - {\normalizedmomentcomp{1}}^2 + \normalizedmomentcomp{2-} + \normalizedmomentcomp{2+}}{\normalizedmomentcomp{2-}\, \normalizedmomentcomp{2+}}}\right)}{\normalizedmomentcomp{2-} + \normalizedmomentcomp{2+}}\\
\normalizedmomentcomp{1-} = \frac{\normalizedmomentcomp{2-}\, \left(\normalizedmomentcomp{1} - \normalizedmomentcomp{2+}\, \sqrt{\frac{ - {\normalizedmomentcomp{1}}^2 + \normalizedmomentcomp{2-} + \normalizedmomentcomp{2+}}{\normalizedmomentcomp{2-}\, \normalizedmomentcomp{2+}}}\right)}{\normalizedmomentcomp{2-} + \normalizedmomentcomp{2+}}
\end{align*}
and $\normalizedmomentcomp{1+}=\normalizedmomentcomp{1-} = 0$ if $\normalizedmomentcomp{2+}=\normalizedmomentcomp{2-} = 0$. In this case, $\distribution = \momentcomp{0}\dirac(\SCheight)$ (due to the quadratic term the second moment vanishes faster than the first moment so we have $\frac{\normalizedmomentcomp{2\pm}}{\normalizedmomentcomp{1\pm}}\to 0$ and $\frac{\normalizedmomentcomp{1\pm}^2}{\normalizedmomentcomp{2\pm}}\to \frac{\normalizedmomentcomp{2\mp}-\normalizedmomentcomp{1}^2}{\normalizedmomentcomp{2\mp}}$). It is simple to check that $\normalizedmomentcomp{1+}+\normalizedmomentcomp{1-} = \normalizedmomentcomp{1}$ and $\cfrac{\normalizedmomentcomp{1+}^2}{\normalizedmomentcomp{2+}}+\cfrac{\normalizedmomentcomp{1-}^2}{\normalizedmomentcomp{2-}} = 1$, i.e. all moments are correctly represented. It remains to show that under \eqref{eq:Realizability1D} we have that $\cfrac{\normalizedmomentcomp{2+}}{\normalizedmomentcomp{1+}}\in[0,1]$ and $\cfrac{\normalizedmomentcomp{2-}}{\normalizedmomentcomp{1-}}\in[-1,0]$, i.e. 
\begin{align*}
0 \leq \normalizedmomentcomp{2\pm} \leq \pm\normalizedmomentcomp{1\pm}.
\end{align*}
This corresponds to the standard half-moment realizability conditions of second order. %This is true if
%\begin{align*}
%\frac{\normalizedmomentcomp{1} + \normalizedmomentcomp{2-}\, \sqrt{\frac{ - {\normalizedmomentcomp{1}}^2 + \normalizedmomentcomp{2-} + \normalizedmomentcomp{2+}}{\normalizedmomentcomp{2-}\, \normalizedmomentcomp{2+}}}}{\normalizedmomentcomp{2-} + \normalizedmomentcomp{2+}} \geq 1\\
% - {\normalizedmomentcomp{1}}^2 + \normalizedmomentcomp{2-} + \normalizedmomentcomp{2+}\geq 0\\
%\pm\normalizedmomentcomp{1\pm}\geq 0
%\end{align*}
We first note that \eqref{eq:Realizability1D}+\eqref{eq:Realizability1Db} imply that $\normalizedmomentcomp{2\pm}\in [0,1]$ since otherwise the bounds become complex. Second, we have that $\normalizedmomentcomp{2+} - \sqrt{\normalizedmomentcomp{2-}\, \left(1-\normalizedmomentcomp{2+}\right)} = \sqrt{\normalizedmomentcomp{2+}\, \left(1-\normalizedmomentcomp{2-}\right)} - \normalizedmomentcomp{2-}$ if and only if $\normalizedmomentcomp{2+} = 1-\normalizedmomentcomp{2-}$ or $\normalizedmomentcomp{2+} = \normalizedmomentcomp{2-} = 0$, implying the classical full-moment realizability conditions $\normalizedmomentcomp{1}\in[-1,1]$ and $\normalizedmomentcomp{2}\leq 1$.

We start the investigation at the different parts of the realizability boundary. Let $\normalizedmomentcomp{1} = \sqrt{\normalizedmomentcomp{2+}\, \left(1-\normalizedmomentcomp{2-}\right)} - \normalizedmomentcomp{2-}$. Plugging this into the definition of $\normalizedmomentcomp{1+}$ we get that, after some elementary transformations,
%
\begin{align*}
\normalizedmomentcomp{1+} &= \cfrac{\normalizedmomentcomp{2+}}{\normalizedmomentcomp{2+}+\normalizedmomentcomp{2-}}\left(\sqrt{1-\normalizedmomentcomp{2-}}\left(\sqrt{\normalizedmomentcomp{2+}}+\cfrac{\normalizedmomentcomp{2-}}{\sqrt{\normalizedmomentcomp{2+}}}\right)\right)\\
&\stackrel{1\geq\normalizedmomentcomp{2+}+\normalizedmomentcomp{2-}}{\geq} \cfrac{\normalizedmomentcomp{2+}}{\normalizedmomentcomp{2+}+\normalizedmomentcomp{2-}}\left(\sqrt{\normalizedmomentcomp{2+}}\left(\sqrt{\normalizedmomentcomp{2+}}+\cfrac{\normalizedmomentcomp{2-}}{\sqrt{\normalizedmomentcomp{2+}}}\right)\right) = \normalizedmomentcomp{2+}.
\end{align*}
Similarly, we obtain $-\normalizedmomentcomp{1-}\geq \normalizedmomentcomp{2-}$ and the same in the case $\normalizedmomentcomp{1} = \normalizedmomentcomp{2+} - \sqrt{\normalizedmomentcomp{2-}\, \left(1-\normalizedmomentcomp{2+}\right)}$.

%We start the investigation at the different parts of the realizability boundary. Let $\normalizedmomentcomp{2+} = 1-\normalizedmomentcomp{2-}$. Then we have $\normalizedmomentcomp{1} = 1-2\normalizedmomentcomp{2-}$ and consequently $\normalizedmomentcomp{1+} = 1-\normalizedmomentcomp{2-}=\normalizedmomentcomp{2+}$, $\normalizedmomentcomp{1-} = -\normalizedmomentcomp{2-}$, i.e. the second-order half-moment realizability conditions are fulfilled with equality.
%
%If $\normalizedmomentcomp{2+} = \normalizedmomentcomp{2-} = 0$ we have $\normalizedmomentcomp{1+} = \normalizedmomentcomp{1-} = 0$ also satisfying the realizability conditions.
%
%Let $\normalizedmomentcomp{2+} > \normalizedmomentcomp{2-} = 0$. Then we have 
%\begin{align*}
%\normalizedmomentcomp{1-} &= 0\\
%\normalizedmomentcomp{1+} &= \normalizedmomentcomp{1} \stackrel{\eqref{eq:Realizability1D}}{\in} [\normalizedmomentcomp{2+},\sqrt{\normalizedmomentcomp{2+}}].
%\end{align*}
%In particular $\normalizedmomentcomp{1+}\geq \normalizedmomentcomp{2+}$. Similar for the case $\normalizedmomentcomp{2-} > \normalizedmomentcomp{2+} = 0$.

Since the realizable set is always convex, the argumentation must also hold in the interior of the above set.


\end{proof}

\begin{figure}[h!]

\begin{center}
\includemovie[poster,toolbar,label=mesh.u3d,text={\externaltikz{Realizability}{\relinput{Images/Realizability}}},
%3Daac=7, 3Droll=0, 3Dc2c=0.000000 1.000000 0.000000, 3Droo=17.114049, 3Dcoo=0 0 0,3Dlights=CAD,]{\linewidth}
3Dviews2=Images/my_views.vws]{2\figurewidth}
{2.3\figureheight}{Images/mesh.u3d}
\end{center}

% \centering
% \caption{Difference of the bounds on $\normalizedmomentcomp{1}$ in the realizable set: $\sqrt{\normalizedmomentcomp{2+}\, \left(1-\normalizedmomentcomp{2-}\right)} - \normalizedmomentcomp{2-}-\left(\normalizedmomentcomp{2+} - \sqrt{\normalizedmomentcomp{2-}\, \left(1-\normalizedmomentcomp{2+}\right)}\right)$.}
\caption{The normalized realizable set for the differentiable mixed-moment basis of order $\momentorder=2$.\\
\textbf{Online version}: Press to activate 3D view ($\x$-axis (red): $\normalizedmomentcomp{2+}$, $\y$-axis (green): $\normalizedmomentcomp{2-}$, $z$-axis (blue): $\normalizedmomentcomp{1}$)}
 \label{fig:Realizability}
\end{figure}
%\movieref[3Dgetview]{mesh.u3d}{Click here!}
%\figref{fig:Realizability} shows the difference of the bounds on the first moment. As already shown in the previous proof, the distance of the bounds is zero only at $\normalizedmomentcomp{2+}=\normalizedmomentcomp{2-}=0$ and $\normalizedmomentcomp{2+}+\normalizedmomentcomp{2-} = 1$.
\figref{fig:Realizability} shows the normalized realizable set (i.e. $\momentcomp{0}=1$), defined by \eqref{eq:Realizability1D} and \eqref{eq:Realizability1Db}.

\begin{remark}
\eqref{eq:Realizability1D} gives a surprising insight into realizability of mixed-moment models. While the realizable set for full-moment and classical mixed-moment models can be characterized by inequalities with rational functions of the moments, the differential mixed-moment model requires non-linearities. This implies that it might be impossible to transfer the general mixed-moment structure (which uses a linearity argument) shown in \cite{Schneider2014} to the differentiable case. 
\end{remark}


==> tikzlibrarynode-families.code.tex <==
\let\tikz@lib@nf@textheight\relax
\let\tikz@lib@nf@textdepth\relax
\let\tikz@lib@nf@textwidth\relax
\tikzset{
  Minimum Width/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@width}{}{%
      \tikzset{/tikz/minimum width/.expand twice=+\csname\pgfpictureid @#1@width\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}\global\let\tikz@lib@nf@outerxsep\tikz@lib@nf@outerxsep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{east}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{west}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \pgfutil@ifundefined{\pgfpictureid @#1@width}{%
              \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@width\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{width}{width}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Height/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@height}{}{%
      \tikzset{/tikz/minimum height/.expand twice=+\csname\pgfpictureid @#1@height\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerysep{\pgfkeysvalueof{/pgf/outer ysep}}\global\let\tikz@lib@nf@outerysep\tikz@lib@nf@outerysep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{north}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{south}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \pgfutil@ifundefined{\pgfpictureid @#1@height}{%
              \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@height\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{height}{height}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Size/.style={
    Minimum Height={#1},
    Minimum Width={#1}},
  Text Height/.code=\edef\tikz@lib@nf@textheight{#1},
  Text Depth/.code= \edef\tikz@lib@nf@textdepth{#1},
  Text Width/.code=%
    \edef\tikz@lib@nf@textwidth{#1}%
    \pgfutil@ifundefined{\pgfpictureid @#1@textwidth}{}{%
      \tikzset{text width/.expand twice=+\csname\pgfpictureid @#1@textwidth\endcsname}%
    }%
}

\def\tikz@lib@nf@text@#1#2#3{%
  \expandafter\ifx\csname tikz@lib@nf@#3\endcsname\relax\else
    \ifx#1\wd\def\tikz@temp{@}\else\let\tikz@temp\pgfutil@empty\fi
    \expandafter\ifx\csname tikz@lib@nf@#3\tikz@temp\endcsname\pgfutil@empty\else
      \pgfutil@ifundefined{\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp}{%
        \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
      }{%
        \ifdim\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname<#1#2
          \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
        \else
          \ifx#1\wd\else
            #1#2=\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\endcsname\relax
          \fi
        \fi
      }%
      \edef\tikz@temp{\noexpand\tikz@lib@nf@save{\pgfpictureid}{\csname tikz@lib@nf@#3\endcsname}{#3}{#3\tikz@temp}}%
      \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
      \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\tikz@temp}%
    \fi
  \fi
}
%%% Redefinition
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    %
    %
    \tikz@lib@nf@text@\ht\pgfnodeparttextbox{textheight}%
    \tikz@lib@nf@text@\dp\pgfnodeparttextbox{textdepth}%
    \tikz@lib@nf@text@\wd\pgfnodeparttextbox{textwidth}%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}
\def\tikz@lib@nf@save#1#2#3#4{%
  \pgfutil@ifundefined{#1@#2@#3@done}{%
    \expandafter\let\csname#1@#2@#3@done\endcsname\pgfutil@empty%
    \immediate\write\pgfutil@auxout{\noexpand\expandafter\noexpand\gdef\noexpand\csname#1@#2@#3\endcsname{\csname#1@#2@#4\endcsname}}
  }{}%
}
\endinput

==> tikzlibrarypositioning-plus.code.tex <==
% This is the TikZ library positioning-plus
% Load with \usetikzlibrary{positioning-plus}
%
% This small library extends TikZ options like 'above', 'left' or 'below right'
% so that they can be used with an optional prefixed factor seperated by ':' (colon)
%
% The option 'left=.5:of somenode' will place
% a new node .5cm (default 'node distance' is '1cm and 1cm') left to (somenode).
% The option 'above right=.2 and .7:of someothernode' will place
% a new node .2cm above and .7cm right of (someothernode).
%
% Additional the options 'xshift*' and 'yshift*' add an additional shift
% as a factor of 'node distance'
% Inspired by http://tex.stackexchange.com/a/117610/16595

\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\pgfdeclaregenericanchor{corner south east}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north east}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner south west}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north west}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}

\tikzset{corner above left/.code=\tikz@lib@place@handle@{#1}{corner south east}{-1}{1}{corner north west}{0.707106781}}
\tikzset{corner above right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{1}{corner north east}{0.707106781}}
\tikzset{corner below left/.code=\tikz@lib@place@handle@{#1}{corner north east}{-1}{-1}{corner south west}{0.707106781}}
\tikzset{corner below right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{-1}{corner south east}{0.707106781}}

\tikzset{corner north left/.code =\tikz@lib@place@handle@{#1}{corner north east}{-1}{0}{corner north west}{1}}
\tikzset{corner north right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{0}{corner north east}{1}}
\tikzset{corner south left/.code =\tikz@lib@place@handle@{#1}{corner south east}{-1}{0}{corner south west}{1}}
\tikzset{corner south right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{0}{corner south east}{1}}

\tikzset{corner west above/.code =\tikz@lib@place@handle@{#1}{corner south west}{0}{1}{corner north west}{1}}
\tikzset{corner west below/.code=\tikz@lib@place@handle@{#1}{corner north west}{0}{-1}{corner south west}{1}}
\tikzset{corner east above/.code =\tikz@lib@place@handle@{#1}{corner south east}{0}{1}{corner north east}{1}}
\tikzset{corner east below/.code=\tikz@lib@place@handle@{#1}{corner north east}{0}{-1}{corner south east}{1}}

\tikzset{north left/.code =\tikz@lib@place@handle@{#1}{north east}{-1}{0}{north west}{1}}
\tikzset{north right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{0}{north east}{1}}
\tikzset{south left/.code =\tikz@lib@place@handle@{#1}{south east}{-1}{0}{south west}{1}}
\tikzset{south right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{0}{south east}{1}}

\tikzset{west above/.code =\tikz@lib@place@handle@{#1}{south west}{0}{1}{north west}{1}}
\tikzset{west below/.code=\tikz@lib@place@handle@{#1}{north west}{0}{-1}{south west}{1}}
\tikzset{east above/.code =\tikz@lib@place@handle@{#1}{south east}{0}{1}{north east}{1}}
\tikzset{east below/.code=\tikz@lib@place@handle@{#1}{north east}{0}{-1}{south east}{1}}

\newif\ifqrr@tikz@lib@place@postransform
\tikzset{node distance transformation/.is if=qrr@tikz@lib@place@postransform}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \ifqrr@tikz@lib@place@postransform
      \pgf@pos@transform{\pgf@x}{\pgf@y}% change from original
    \fi
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \pgfutil@in@{:}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@#1\tikz@stop
    \ifx\pgf@temp\pgfutil@empty
      \let\pgf@temp\tikz@node@distance
    \fi
    \pgfmathsetmacro\pgf@tempa{(\pgf@tempa)*#4}%
    \pgfmathsetmacro\pgf@tempb{(\pgf@tempb)*#3}%
    \edef\pgf@marshal{\noexpand\tikz@lib@place@handle@{\pgf@temp}{#2}{\pgf@tempb}{\pgf@tempa}{#5}{#6}}%
    \pgf@marshal
  \else
    \def\tikz@anchor{#2}%
    \let\tikz@do@auto@anchor=\relax%
    \edef\tikz@temp{#1}%
    \def\tikz@lib@place@single@factor{#6}%
    \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
  \fi
}
\def\tikz@lib@place@handle@qrr@#1:#2\tikz@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@@#1\tikz@stop
  \else
    \tikz@lib@place@handle@qrr@@#1and#1\tikz@stop
  \fi
  \def\pgf@temp{#2}%
}
\def\tikz@lib@place@handle@qrr@@#1and#2\tikz@stop{%
  \def\pgf@tempa{#1}%
  \def\pgf@tempb{#2}%
}
\def\qrr@xyshift@starred#1#2#3{
  \edef\tikz@marshal{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
  \tikz@marshal
  \ifpgfutil@in@
    \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
  \else
    \let#3\tikz@node@distance
  \fi
  \pgfmathparse{(#1)*#3}%
  \ifpgfmathunitsdeclared
    \if#2x%
      \pgftransformshift{\pgfqpoint{\pgfmathresult pt}{0pt}}%
    \else
      \pgftransformshift{\pgfqpoint{0pt}{\pgfmathresult pt}}%
    \fi
  \else
    \ifx#2x
      \pgf@process{\pgfqpointxy{\pgfmathresult}{0}}%
    \else
      \pgf@process{\pgfqpointxy{0}{\pgfmathresult}}%
    \fi
    \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi}
\tikzset{
  xshift*/.code=\qrr@xyshift@starred{#1}x\pgf@tempb,
  yshift*/.code=\qrr@xyshift@starred{#1}y\pgf@tempa,
}

\def\pgfutil@firstofmany#1#2\pgf@stop{#1}
\def\pgfutil@secondofmany#1#2\pgf@stop{#2}
\def\tikz@lib@place@of@#1#2#3{%
  \def\pgf@tempa{fit bounding box}%
  \edef\pgf@temp{\expandafter\pgfutil@firstofmany#2\pgf@stop}
  \if\pgf@temp(%
    \tikz@lib@place@fit@scan{#2}{0}%
  \else\if\pgf@temp|
      \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
    \else\ifx\pgf@temp\tikz@activebar
        \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
      \else\if\pgf@temp-
          \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{2}%
        \else\if\pgf@temp+
            \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{3}%
          \else
            \def\pgf@tempa{#2}%
          \fi
        \fi
      \fi
    \fi
  \fi
  \expandafter\tikz@scan@one@point\expandafter\tikz@lib@place@remember\expandafter(\pgf@tempa)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@fit@scan#1#2{
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  \if\pgfutil@firstofmany#1\pgf@stop(%
    \tikz@lib@fit@scan#1\pgf@stop%
  \else
    \tikz@lib@fit@scan(#1)\pgf@stop
  \fi
  \ifdim\pgf@xa>\pgf@xa
    % shouldn't happen
  \else
     \expandafter\def\csname pgf@sh@ns@fit bounding box\endcsname{rectangle}%
     \expandafter\edef\csname pgf@sh@np@fit bounding box\endcsname{%
       \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
       \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
     }%
     \expandafter\def\csname pgf@sh@nt@fit bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
     \expandafter\def\csname pgf@sh@pi@fit bounding box\endcsname{\pgfpictureid}%
     \ifcase#2\relax
     \or % 1 = vertical
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})}}}%
       \pgf@marshal
     \or % 2 = horizontal
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \or % 3 = both directions
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})},minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \fi
  \fi
}
\tikzset{
  fit bounding box/.code={\tikz@lib@place@fit@scan{#1}{0}},
  span vertical/.code={\tikz@lib@place@fit@scan{#1}{1}},
  span horizontal/.code={\tikz@lib@place@fit@scan{#1}{2}},
  span/.code={\tikz@lib@place@fit@scan{#1}{3}}}

\pgfmathdeclarefunction{x_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempb}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
\pgfmathdeclarefunction{y_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempa}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
%\tikzdeclarecoordinatesystem{node distance}{%
%  \tikz@cs@nd#1\tikz@stop}
%\def\tikz@cs@nd#1,#2\tikz@stop{%
%  \def\qrr@xyshift@starred@action##1{\pgftransformshift{##1}}%
%  \qrr@xyshift@starred{#1}x\pgf@tempb
%  \qrr@xyshift@starred{#2}y\pgf@tempa}
\endinput
